Large Language Models are Skeptics: False Negative Problem of Input-conflicting Hallucination

In this paper, we identify a new category of bias that induces input-conflicting hallucinations, where large language models (LLMs) generate responses inconsistent with the content of the input context. This issue we have termed the false negative problem refers to the phenomenon where LLMs are predisposed to return negative judgments when assessing the correctness of a statement given the context. In experiments involving pairs of statements that contain the same information but have contradictory factual directions, we observe that LLMs exhibit a bias toward false negatives. Specifically, the model presents greater overconfidence when responding with False. Furthermore, we analyze the relationship between the false negative problem and context and query rewriting and observe that both effectively tackle false negatives in LLMs.

==> section/3.Method.tex <==
\section{Context and Statement Rewriting and False Negative Problem}\label{sec:chain_of_question}

In this section, we analyze the impact of context and statement rewriting on the false negative problem.
In the remaining text, we describe processes focusing on the question answering task where the question $q$ in the statement is the only target to be rewritten.
The term \textit{question} can be replaced with \textit{statement} for the general case.

For each rewriting process, we introduce question-based context filtering (QCF) and iterative answer refinement (IAR).
Both QCF and IAR aim to map the context and question into a distribution of high likelihood that makes it easier for LLMs to discriminate the factuality of the statement.
Furthermore, QCF ensures that the facts related to the question within the context are dense.

In all the processes of QCF and IAR, the same LLM without any fine-tuning as used in the experiment is employed, proceeding with zero-shot prompting. 
Detailed prompts for each process can be found in Table \ref{table:prompt_details} of Appendix \ref{appendix:details_on_prompts}.

\begin{table*}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 & \multicolumn{4}{c|}{All} & \multicolumn{4}{c|}{Parametric} & \multicolumn{4}{c|}{Counterfactual} \\
\hline
 & \multicolumn{2}{c|}{All-True} & \multicolumn{2}{c|}{All-False} & \multicolumn{2}{c|}{All-True} & \multicolumn{2}{c|}{All-False} & \multicolumn{2}{c|}{All-True} & \multicolumn{2}{c|}{All-False} \\
\hline
 & FN & FN/(TP+FN) & FP & FP/(TN+FP) & FN & FN/(TP+FN) & FP & FP/(TN+FP) & FN & FN/(TP+FN) & FP & FP/(TN+FP) \\
\hline
Mistral & 1052 & \textbf{0.565} & 510 & 0.268 & 381 & \textbf{0.438} & 237 & 0.189 & 611 & 0.671 & 255 & 0.418 \\
+ QCF & 986 & 0.574 & 516 & 0.293 & 382 & 0.490 & 272 & 0.233 & 593 & 0.649 & 240 & 0.412 \\
+ IAR & \textbf{876} & 0.585 & \textbf{375} & \textbf{0.239} & \textbf{345} & 0.514 & \textbf{184} & \textbf{0.183} & \textbf{522} & \textbf{0.643} & \textbf{187} & \textbf{0.344} \\
\hline
ChatGPT & 1068 & 0.468 & 509 & 0.223 & 72 & 0.102 & \textbf{253} & \textbf{0.131} & 994 & 0.632 & 252 & 0.735\\
+ QCF & 918 & 0.401 & 564 & 0.247 & \textbf{60} & \textbf{0.085} & 312 & 0.163 & 857 & 0.543 & 246 & 0.685\\
 + IAR & \textbf{875} & \textbf{0.382} & \textbf{489} & \textbf{0.214} & 109 & 0.154 & 310 & 0.162 & \textbf{764} & \textbf{0.484} & \textbf{175} & \textbf{0.486}\\
\hline
GPT-4 & \textbf{585} & \textbf{0.259} & 411 & 0.181 & \textbf{157} & \textbf{0.107} & 155 & 0.086 & \textbf{427} & \textbf{0.538} & 256 & 0.552\\
+ QCF & 693 & 0.295 & 357 & 0.156 & 249 & 0.169 & 133 & 0.073 & 444 & 0.552 & 224 & 0.479\\
 + IAR & 1029 & 0.451 & \textbf{235} & \textbf{0.103} & 495 & 0.335 & \textbf{97} & \textbf{0.053} & 486 & 0.666 & \textbf{138} & \textbf{0.296}\\
\hline
\end{tabular}}
\caption{
False positives (FPs) and false negatives (FNs) results of QCF and IAR on All-True and All-False prompts. TP and TN denote true positive and true negative, respectively.
}\label{table:all_true_and_all_false}
\end{table*}

\subsection{Question-based Context Filtering}
In typical retrieval-augmented generation scenarios, the raw context becomes lengthy, making the facts in the context necessary for factuality discrimination sparse. 
To address this issue, QCF involves processes of question decomposition and fact extraction followed by fact reorganization.

\textbf{Sub-question Generation} Questions are often complex or require multi-step reasoning. 
Considering this, we first use the LLM to divide the question into multiple sub-questions.
We follow the question decomposition prompt in DDCoT (\citealp{zheng-2023-ddcot}).
Through question decomposition, we aim to facilitate the collection of relevant facts.
For example, for the question \textit{"Are more people today related to Genghis Khan than to Julius Caesar?"}, the generated sub-questions aim to collect facts related to the number of people associated with or descended from Genghis Khan and Julius Caesar, as illustrated in Figure \ref{fig:overview} (a).

\textbf{Question-based Fact Extraction} We then use each sub-question and the context to prompt the LLM to extract the necessary facts from the context. 
Finally, in the fact reorganization process, we prompt the LLM to filter and reorder the extracted facts to construct a filtered context $c'$ using the original question.

\subsection{Iterative Answer Refinement}\label{subsec:iterative_answer_refinement}
\textbf{Context-based Question Rewriting} In IAR, we first rewrite the question $n$ times based on the context $c'$.
The goal of this process is to obtain a statement that is easier for the LLM to understand and ground in the given context.
We denote the rewritten questions including the original one as $Q=\{q_0, q_1, q_2, ..., q_n\}$, where $q_0=q$.
In Figure \ref{fig:overview} (b), for instance, the question is incrementally paraphrased by the LLM into a distribution with a high likelihood, where $n$ is 3.

\textbf{Final Prediction} Using the question $q$, filtered context $c'$, and rewritten questions $Q$, we proceed with conversation-style factuality discrimination.
Initially, we input $q_n$ and $c'$ into the LLM to obtain the prediction $a_n$. 
In the $i$-th step, we input $q_{n-i}$, $c'$, and the dialog history $D_i=\{(q_n, a_n), ..., (q_{n-i+1}, a_{n-i+1})\}$ into the LLM to derive $a_{n-i}$.
Finally, we input the original question $q$ for the statement, along with $c'$ and $D=D_n$, into the LLM to obtain the final factuality prediction.

Figure \ref{fig:overview} assumes the Original prompt setting, and note that in All-True and All-False prompt settings, the final question is converted into statement form.


==> section/4.Results.tex <==
\section{Experiments}\label{sec:experiments}

\subsection{Setting}
During the sub-question generation step, the LLM is prompted to generate no more than five sub-questions to minimize redundancy. 
In the question-based fact extraction step, facts are collected by iteratively inputting each sub-question and concatenated. 
We filter out null responses (e.g., “There is no information related to the question.”) during the fact extraction.
In the context-based question rewriting stage, the number of iterations $n$ is set to 5 as a default. 
In all the stages except the IAR stage, the temperature during decoding is set to 1.0, and the temperature during answering is set to 0.0.

All the models are prompted to answer the question with True or False.
The prediction is classified as Unknown only in the cases where neither True nor False exists in the prediction.
% We set the maximum length of the generated tokens to 256 for sub-question generation, 512 for question-based fact extraction, and 1024 for fact filtering and reordering.



% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=0.93\textwidth]{figures/figure3.pdf}
%     \caption{The ratio of false positives (FPs) in All-False prompt and false negatives (FNs) in All-True prompt according to the number of question rewritings in Mistral and ChatGPT.}
%     \label{fig:n_study}
% \end{figure*}


\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.93\textwidth]{figures/figure4.v4.pdf}
    \caption{Histogram of Mistral based on the confidence of predicted labels for counterfactual samples in the All-True (Top) and All-False (Bottom) prompt. Baseline refers to the Mistral without QCF and IAR, and $n$ indicates the number of question rewritings after QCF.}
    \label{fig:confidence_histogram}
\end{figure*}

\subsection{Main Results}
\subsubsection{Results on All-True and All-False Prompts}
Table \ref{table:all_true_and_all_false} shows the ratios and numbers of false positives/negatives among valid predictions for All-True/False prompts, respectively. 
In Mistral and ChatGPT, QCF and IAR effectively reduce false positives and negatives. 
Notably, there is a significant decrease in discrimination errors for counterfactual samples, where the false negative problem mainly occurs. 
However, in parametric samples, the change in false positives/negatives due to QCF and IAR is less compared to counterfactual cases.

QCF and IAR on GPT-4 significantly increase false negatives, leading to a greater discrepancy in accuracy between All-True and All-False prompts.
In our observations, we have noted that GPT-4 tends to return a null response during the fact extraction in QCF and the conversation-style factuality discrimination in IAR processes.

The null response in the fact extraction process results in the filtered context becoming insufficient or empty, leading to a sharp increase in "False" predictions for given statements.
On the other hand, in the process of conversation-style factuality discrimination, the occurrence of even a single null response leads to the final prediction being concluded as "False".
% The reason for the different behavior of GPT-4 compared to other LLMs should be investigated in future work.
% We observe that during the fact extraction and final prediction processes, GPT-4 tends to return a null response instead of partial evidence. 
% The null response tendency of GPT-4 significantly increases the cases where the filtered context is insufficient or empty, leading to a sharp increase in false negatives in response to given statements.

\begin{table}[!t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
\hline
 & \multicolumn{3}{c|}{All} & \multicolumn{3}{c|}{Parametric} & \multicolumn{3}{c|}{Counterfactual} \\
\hline
 & FN & FP & Unk. & FN & FP & Unk. & FN & FP & Unk. \\
\hline
Mistral & 487 & \textbf{120} & 532 & 4 & \textbf{37} & 124 & 199 & 7 & 100 \\
+ QCF & 402 & 189 & 778 & 8 & 83 & 182 & 163 & 5 & 140 \\
+ IAR & \textbf{166} & 206 & 1378 & \textbf{2} & 119 & 402 & \textbf{57} & \textbf{4} & 235 \\
\hline
ChatGPT & 614 & \textbf{77} & 3 & 62 & \textbf{38} & 2 & 551 & \textbf{39} & 1 \\
+ QCF & 554 & 107 & 2 & 53 & 66 & 2 & 500 & 41 & 0\\
 + IAR & \textbf{435} & 228 & 44 & \textbf{51} & 178 & 28 & \textbf{384} & 50 & 16 \\
\hline
GPT-4 & 324 & \textbf{93} & 202 & 58 & \textbf{34} & 92 & 196 & 43 & 29 \\
+ QCF & \textbf{293} & 107 & 186 & \textbf{46} & 41 & \textbf{78} & 186 & 47 & 21 \\
 + IAR & 310 & 101 & 310 & 79 & 51 & 149 & \textbf{164} & \textbf{37} & 55 \\
\hline
\end{tabular}}
\caption{
Results of QCF and IAR in the Original prompt setting. FP, FN, and Unk. denote false positives, false negatives, and Unknown, respectively.
}\label{table:original_prompt}
\end{table}


\subsubsection{Results on Original Prompt}
Table \ref{table:original_prompt} shows the number of false positives, false negatives, and unknown responses in the Original prompt setting. 
As with the All-True and All-False prompts, QCF and IAR mitigate the false negative problem in counterfactual samples. 
This means that mitigating the false negative problem in the All-True/All-False leads to alleviating the issue in the original question answering scenario.
Interestingly, for all samples of the three models, both QCF and IAR increase the occurrence of Unknown. 
We hypothesize that the phenomenon is due to changes in the prediction confidence and conduct analysis in Section \ref{sec:analysis}.

As seen in Tables \ref{table:all_true_and_all_false} and \ref{table:original_prompt}, there is a greater change in the number of false positives/negatives at IAR than QCF. 
In other words, iterative answer refinement is more effective in addressing the false negative problem compared to context filtering.




==> section/Ethics_Statement.tex <==
\section{Ethics Statement}\label{sec:ethics_statement}
